On Constant-Round Concurrent Zero-Knowledge from a Knowledge Assumption

In this work, we consider the long-standing open question of constructing constant-round concurrent zero-knowledge protocols in the plain model. Resolving this question is known to require non-black-box techniques. We consider non-black-box techniques for zero-knowledge based on knowledge assumptions, a line of thinking initiated by the work of Hada and Tanaka (CRYPTO 1998). Prior to our work, it was not known whether knowledge assumptions could be used for achieving security in the concurrent setting, due to a number of significant limitations that we discuss here. Nevertheless, we obtain the following results: 1. We obtain the first constant round concurrent zero-knowledge argument for \textbf{NP} in the plain model based on a new variant of knowledge of exponent assumption. Furthermore, our construction avoids the inefficiency inherent in previous non-black-box techniques such that those of Barak (FOCS 2001); we obtain our result through an efficient protocol compiler. 2. Unlike Hada and Tanaka, we do not require a knowledge assumption to argue the soundness of our protocol. Instead, we use a discrete log like assumption, which we call Diffie-Hellman Logarithm Assumption, to prove the soundness of our protocol. 3. We give evidence that our new variant of knowledge of exponent assumption is in fact plausible. In particular, we show that our assumption holds in the generic group model. 4. Knowledge assumptions are especially delicate assumptions whose plausibility may be hard to gauge. We give a novel framework to express knowledge assumptions in a more flexible way, which may allow for formulation of plausible assumptions and exploration of their impact and application in cryptography.

==> commitmentdl.tex <==
\subsection{Discrete Log based Equivocal Commitment Scheme \comdl}
\label{commitdl}
The committer and the receiver are given a group $\mathbb{G}$ of prime order $q$, its generator $g$ and an element $B \in \mathbb{G}$ such that $q$ is an $n-$bit prime. To commit to $x \in \mathbb{Z}_q$, choose $r \xleftarrow{\$} \mathbb{Z}_q$ and send $Z = g^x\cdot B^r$. To open, the sender sends $(x,r)$. 

This commitment scheme is perfectly hiding i.e. $\comdl(x)$ and $\comdl(x')$ are identically distributed. If the committer does not know the discrete log of $B$, then $\comdl$ is computationally binding under discrete log assumption. \red{We assume that discrete log assumption holds in all the groups we consider.} Also, if $Z$ is a commitment under $\comdl$, then given two distinct openings of $Z$ to $(x,r)$ and $(x',r')$ such that $x\ne x'$, one can easily solve for the discrete log of $B$, say $b$, as follows: $b = (x-x')\cdot(r'-r)^{-1}$. Also, if the simulator knows the discrete log of $B$, say $b$, it can open $Z = \comdl(x;r)$\ as being a commitment to any $x' \in \mathbb{Z}_q$ by sending $r' = \comopendl(x, x', r, b) =  (x+r\cdot b - x')\cdot b^{-1}$. 



==> keaux.tex <==
\section{Discussion regarding use of auxiliary inputs for concurrent simulation}
\label{app:KEAUX}


A potentially promising idea for using \ka s for concurrent simulation is the following: Formulate a \ka\ that holds for all auxiliary inputs for the adversary, and then invoke the knowledge extractor provided by the \ka\ with different auxiliary inputs corresponding to the extraction history. In other words, one could attempt to apply a single extractor iteratively for different concurrent sessions, passing along all the information extracted so far as auxiliary input to the extractor.

However, similar to the example discussed in the Introduction concerning a potential ``interactive'' \ka, a problem may arise if the auxiliary input contains ``external knowledge'' and thereby prevents extraction. We stress there is an important distinction between why this fails and failure of the interactive knowledge assumption. Here we are not saying that a \ka\ which holds with regard to all auxiliary inputs must be false. Rather we are saying that any natural application of such an assumption to the concurrent setting would fail.  This is because it would cause us to invoke the extractor with auxiliary inputs that impermissibly correlate with messages received by the adversary in earlier executions of \kcp. By the definition of auxiliary input, an extractor would not be required to function in such a case. To make the intuition precise, consider an example of such an iterative application of knowledge assumption in the concurrent setting. Suppose the Adversary schedules the messages of the malicious committer (MC) as follows: First, MC asks for the random first message of the Receiver (R) in the \kcp\ for all the sessions ($r_1,r_2,\ldots,r_m$). Now, MC chooses a function $f$ and completes the first \kcp\ by committing to $f(r_1,r_2,\ldots,r_m)$. We apply the knowledge assumption to recover $f(r_1,r_2,\ldots,r_m)$. Next, the MC completes another \kcp. Now in order to extract, we need to provide the extractor one of the random $r_i$'s as input and $f(r_1,r_2,\ldots,r_m)$ as auxiliary input. But here, depending on the function $f$, this auxiliary input may be highly correlated to the input $r_i$.  In this case, the extractor is \emph{allowed} to fail with high probability.
This is because the extractor is only required to work for the fixed auxiliary input $aux = f(r_1, r_2, \dots, r_m)$, when $r_i$ is chosen at random independently of $aux$.  However, the actual simulation would use $aux$ that correlates with the input $r_i$.  


==> related.tex <==
\section{Related Work}
\label{Sec:RW}
\textbf{Knowledge Assumptions} Knowledge or extractability assumptions capture our belief that certain computational tasks can be done efficiently only by going through certain specific intermediate stages and generating some specific kinds of intermediate values. One such class of assumptions is Knowledge of Exponent Assumptions which were first introduced by Damgard~\cite{Dam92} to construct a CCA secure encryption scheme. Though these assumptions do not fall in the class of falsifiable class of assumptions~\cite{Naor03}, these have been proven secure against generic algorithms~\cite{Nechaev94,Shoup97,Dent06}, thus offering some evidence of validity. Hada and Tanaka~\cite{HT98} gave a three round zero-knowledge protocol using two knowledge of exponent assumptions. Later, Bellare and Pallacio~\cite{BP04} proved that the assumption used for proving the soundness of the protocol was false, proposed a modified assumption and recovered the earlier result. We stress that in our protocol, we are able to argue soundness directly without the use of any knowledge assumption. 

Extending the assumption of~\cite{BP04}, Abe and Fehr~\cite{AF07} constructed the first perfect NIZK for NP with full adaptive soundness. Under knowledge of exponents assumption, Prabharakaran and Xue~\cite{PX09} constructed statistically hiding sets based on trapdoor DDH groups~\cite{DG06}. Gennaro et al.~\cite{GKR10} modify the Okamoto-Tanaka key agreement protocol to get perfect forward secrecy. Recently, Groth~\cite{Groth10} generalized the assumption of~\cite{AF07} to short non-interactive perfect zero-knowledge arguments for circuit satisfiability.

Other set of knowledge assumptions used recently are extractable functions~\cite{CD08,CD09}. All of ~\cite{BCCT12,DFH12,GLR11} give one of the constructions of Extractable Collision Resistant Hash functions (ECRH) using Knowledge of Exponent Assumptions. Then assuming the existence of ECRH, Bitansky et al~\cite{BCCT12} modify the construction of~\cite{DCL08} and prove that the modified construction is a succinct non-interactive adaptive arguments of knowledge (SNARK). They also show that existence of SNARKs imply the existence of (their notion of) ECRH. In the CRS model, they combined NIZK and SNARKs to give zero-knowledge non-interactive arguments. On the other hand, Damgard et al~\cite{DFH12} also use ECRH to construct succinct non-interactive arguments in CRS model. Using these, they give a two message protocol for two party computation which is UC-secure. 

\textbf{Concurrent Zero-Knowledge:} The difficulty in constructing a round-efficient $c\mathcal{ZK}$ was first observed by Dwork et al.~\cite{DNA98}. Following this, rigorous lower bounds on round complexity of $c\mathcal{ZK}$ for NP with a black-box simulator have been proven in~\cite{KPR98,Rosen00,CKPR01}; the best lower bound being $\Omega(\log n/\log \log n)$ rounds given by Canetti et al.~\cite{CKPR01}. \\
Barak~\cite{Barak01} gave a constant round protocol for all NP, in which he gave a non-black-box simulator for zero-knowledge. Also, for any predetermined polynomial $p(\cdot)$, this constant round protocol is zero-knowledge even when $p(n)$ sessions are concurrently executed. But it has a major drawback. The polynomial $p(\cdot)$ has to be fixed at the beginning of the protocol and the message lengths grow linearly in $p(n)$. Killian and Petrank~\cite{KP01} gave a poly-logarithmic round protocol which is zero-knowledge even when it is executed concurrently for any (not determined) polynomial number of times. The gap between the upper and lower bounds of round complexity of black-box $c\mathcal{ZK}$ was closed by Prabhakaran, Rossen, and Sahai~\cite{PRS02} who gave a $\tilde{O}(\log n)$ round protocol. Since then improving the round complexity of concurrent zero-knowledge has been an open problem.

